Resolving Oversmoothing with Opinion Dissensus

While graph neural networks (GNNs) have allowed researchers to successfully apply neural networks to non-Euclidean domains, deep GNNs often exhibit lower predictive performance than their shallow counterparts. This phenomena has been attributed in part to oversmoothing, the tendency of node representations to become increasingly similar with network depth. In this paper we introduce an analogy between oversmoothing in GNNs and consensus (i.e., perfect agreement) in the opinion dynamics literature. We show that the message passing algorithms of several GNN models are equivalent to linear opinion dynamics models which have been shown to converge to consensus for all inputs regardless of the graph structure. This new perspective on oversmoothing motivates the use of nonlinear opinion dynamics as an inductive bias in GNN models. In our Behavior-Inspired Message Passing (BIMP) GNN, we leverage the nonlinear opinion dynamics model which is more general than the linear opinion dynamics model, and can be designed to converge to dissensus for general inputs. Through extensive experiments we show that BIMP resists oversmoothing beyond 100 time steps and consistently outperforms existing architectures even when those architectures are amended with oversmoothing mitigation techniques. We also show that BIMP has several desirable properties including well behaved gradients and adaptability to homophilic and heterophilic datasets.

==> sections/3_preliminaries.tex <==
In this section we describe our notation and review nonlinear opinion dynamics~\cite{leonard2024fast}.
%
Throughout this text we use lower-case letters for scalar valued variables, boldface lower-case letters for vectors, and boldface upper-case letters for matrices. 
% For a matrix $\mathbf{X}$, we denote its $i$-th column as $\mathbf{x}_i$. 
% We define graphs as the set $\mathcal{G}=(\mathcal{V},\mathcal{E})$ with $n=|\mathcal{V}|$ nodes and $m=|\mathcal{E}|$. 
% For multi-agent system evolving under opinion dynamics models we use $N_\mathrm{a}$ to denote the number of agents and $N_\mathrm{o}$ to denote the number of options.

\subsection{Nonlinear opinion dynamics}
Nonlinear opinion dynamics captures the evolution of agent opinions in a multi-agent system. Opinions for each option can be positive, neutral, or negative, where the magnitude correlates to the opinion strength. Changes to these opinions are affected by extrinsic and intrinsic parameters. Specifically, agent $i$'s opinion about option $j$ can be described by the following nonlinear differential equation proposed in~\cite{ bizyaeva2022nonlinear, leonard2024fast},
%
\begin{equation}
    \dot{x}_{ij} = -d_{ij}x_{ij} + S\Bigg(u_i \Bigg( \alpha^j_i x_{ij} + \sum^{N_\mathrm{a}}_{\substack{k=1 \\ k \neq i}}a^{\mathrm{a}}_{ik}x_{kj} + \sum^{N_\mathrm{o}}_{\substack{l=1\\ l\neq j}}a^{\mathrm{o}}_{jl}x_{il} + \sum^{N_\mathrm{a}}_{\substack{k=1 \\ k \neq i}} \sum^{N_\mathrm{o}}_{\substack{l=1 \\ l \neq j}} a^{\mathrm{a}}_{ik} a^{\mathrm{o}}_{jl} x_{kj}\Bigg) \Bigg) + b_{ij} \label{eq:nod}.
\end{equation}
%
The parameters $d_{ij}\geq0$, $u_{i}>0$, and $\alpha_{i}^{j}\geq0$ are intrinsic to each agent. The damping term $d_{ij}$ describes the resilience of agent $i$ to forming an opinion on option $j$; the attention $u_{i}$ represents the attentiveness of agent $i$ to the opinions of other agents; and the self-reinforcement $\alpha_{i}^{j}$ defines the resistance of agent $i$ to changing the opinion for option $j$.

The parameters $a^{\mathrm{a}}_{jk}$, $a^{\mathrm{o}}_{jl}$, and $b_{ij}$, and saturating function $S\left(\cdot\right)$ are extrinsic to the agents. The environmental $b_{ij}$ represents the impact of the environment on the agent's opinion for option $j$. The saturating function $\mathcal{S}$ is selected so that  $S\left(0\right)=0$, $S'\left(0\right)=1$, and $S'''\left(0\right)\neq0$. We use a hyperbolic tangent for the saturation function in our method.

The communication network graph $\mathcal{G}^\mathrm{a} = (\mathcal{V}^\mathrm{a},\mathcal{E}^\mathrm{a},\mathbf{A}^\mathrm{a})$ describes how agents are able to exchange their opinions over time. The communication adjacency matrix $\mathbf{A}^{\mathrm{a}}=\left[a^{\mathrm{a}}_{ik}\right]\in\mathbb{R}^{N_{\mathrm{a}}\times N_{\mathrm{a}}}$ defines the communication strength between agent $i$ and agent $k$. Similarly, the belief system graph $\mathcal{G}^\mathrm{o} = \left(\mathcal{V}^\mathrm{o}, \mathcal{E}^\mathrm{o}, \mathbf{A}^\mathrm{o}\right)$ describes the correlation between options. The belief adjacency matrix $\mathbf{A}^\mathrm{o}=[a^{\mathrm{o}}_{jl}]\in\mathbb{R}^{N_{\mathrm{o}}\times N_{\mathrm{o}}}$ defines the strength of correlation between option $j$ and $l$.

%The third graph is the \textit{attention} system graph  $\mathcal{G}_u = (\mathcal{V}_u,\mathcal{E}_u,A_u)$. Similarly, we define attention adjacency matrix $A_u=[a^{\mathrm{u}}_{ik}]  \in \mathbb{R}^{N_\mathrm{a}\times N_\mathrm{a}}$ to quantify the strength of agent $k$'s opinion about any option has on agent $i$. Usually, if the agent updates its attention using observations from the communication network, the attention adjacency matrix $A_u$ equals $A_a$.


==> sections/n_backup.tex <==
\newpage
{
\color{blue}
\begin{proof}
Here we provide the proof that time-vary linear opinion dynamics preserves consensus property inspired by \cite{blondel2005convergence}.
Consider a multi-agent system with communication graph $\mathcal{G}^{\mathrm{a}}$, whose dynamics are governed by the discrete-time dynamics defined in Equation \ref{eq:lod}). After $t$ times evolution, we have this form
\begin{equation}
    \dot{\mathbf{X}}(t) = \mathbf{A}(t)\mathbf{A}(t-1) \cdots \mathbf{A}(0)\mathbf{X}(0)
\end{equation}
where each adjacency matrices $\mathbf{A}(t) = [a_{ij}(t)]$ are right stochastic and time-dependent.

In view of the preceding, the dynamics involve opinion exchange among agents only, without interaction among option (i.e., $\mathcal{G}^{\mathrm{o}}=\mathbf{0}$). Therefore, without lack of generality, we focus on the case where individual agent opinions $\mathbf{x}_i$ are scalars, denoted by $x_i$, implying that the opinion dimension is 1. Accordingly, $\mathbf{x} \in \mathbb{R}^{n\times 1}$ now denotes the vector of all agent opinions.

We firstly make two assumptions.
\begin{assumption}[Connectivity]
The graph $\mathcal{G}^{\mathrm{a}}$ is strongly connected and has fixed connectivity. (A1)
\end{assumption}
\begin{assumption}[Uniform Positivity]
    There exists $\zeta > 0$ such that for all $t$, if $a_{ij}(t) > 0$, then $a_{ij}(t) \geq \zeta$. (A2)
\end{assumption}

\begin{lemma}\label{lemma:A1}
    Based on assumption (A1), there exists a path from some agent $k$ to both agent $i$ and agent $j$ within $n-1$ steps.
\end{lemma}
\begin{lemma}\label{lemma:A2}
    Based on lemma \ref{lemma:A1} and assumption (A2), the total influence from $k$ to both $i$ and $j$ doesn't vanish over those steps.
\end{lemma}
We then make two definitions.
\begin{definition}[Minimum and Maximum Agent Opinions]
The minimum and maximum agent opinions are defined as
\begin{equation}
    m(t) = \min \left( \mathbf{x}(t) \right), \;\;\; M(t) = \max \left( \mathbf{x}(t) \right). 
\end{equation}
\end{definition}
\begin{definition}[Diameter]
The diameter of the agent opinions at time $t$ is defined as
    \begin{equation}
    D(t) = M(t) - m(t) \geq 0.
    \end{equation}
\end{definition}

\textbf{Monotonicity of Extremes.} Given the right stochastic property of $\mathbf{A}(t)$, we have
\begin{equation}
\begin{split}
    M(t+1) &= \max \mathbf{A}(t) \mathbf{x}(t) = \max_i \sum_{j=1}^n a_{ij}x_j(t) \leq \max_i \sum_{j=1}^n a_{ij} \max_j x_{j}(t) = \max (\mathbf{x}(t)), \\
    m(t+1) &= \min \mathbf{A}(t) \mathbf{x}(t) = \min_i \sum_{j=1}^n a_{ij}x_j(t) \geq \min_i \sum_{j=1}^n a_{ij} \min_j x_{j}(t) = \min (\mathbf{x}(t)). 
\end{split}
\end{equation}
\begin{lemma}
   $M(t)$ is non-increasing and $m(t)$ is non-decreasing. Therefore, $x(t) \in [m(0), M(0)]$, and $D(t)$ is non-increasing. 
\end{lemma}

Our goal is to show that the diameter is not only non-increasing over time, but also converges to zero asymptotically, as
\begin{equation}
    \lim_{t \to \infty} D(t) = 0.
\end{equation}

% Let $\Phi (t,t+T) = \mathbf{A}(t+T-1)\cdots \mathbf{A}(t)$. Then we have
% \begin{equation}
%     \mathbf{x}(t+T) = \Phi(t,t+T)\mathbf{x}(t)
% \end{equation}
% Given the assumption A1 and A2, we conclude there exist a step interval $\tilde{T}$ that for every $t$, $\Phi(t,t+T)$ is \textbf{scrambling}:
% \begin{equation}
%     \Phi_{ij}(t,t+\tilde{T}) \geq \alpha,\;\;\; \Phi_{kj}(t,t+\tilde{T}) \geq \alpha
% \end{equation}
% which means there’s at least one agent ($j$) that both agents ($i$ and $k$) communicate with directly.

% We have
% \begin{equation}
%     x_i(t+\tilde{T}) = \sum_{k=1}^{n} \Phi_{ik}(t,t+\tilde{T}) x_k(t)
% \end{equation}
% So


% \begin{equation}
%     x_i(t+\tilde{T}) = \sum_{k=1}^{n} \Phi_{ik}(t,t+\tilde{T}) x_k(t)
% \end{equation}

\textbf{Scrambling Property. }Let $T = n-1$, and $\Phi (t) := \mathbf{A}(t+T-1)\cdots \mathbf{A}(t)$. Then we have
\begin{equation}
    \mathbf{x}(t+T) = \Phi(t)\mathbf{x}(t)
\end{equation}
\begin{lemma}\label{lemma:scrambling}
    Under Assumptions (A1) and (A2), we conclude that that for any $t$, $\Phi(t)$ is \textbf{scrambling}, i.e., for any pair $i,k \in \mathcal{E}$, there exists $j$ such that
    \begin{equation}\label{eq:scrambling}
        \Phi_{ij}(t) >0,\;\;\; \Phi_{kj}(t) > 0, \;\;
    \end{equation}
    where $\Phi_{ij}(t)$ denotes the entry of $\Phi(t)$ at row $i$ and column $j$.
    Moreover, there exists $\delta >0$, which depends on $\zeta, n$ and the graph structure, such that:
    \begin{equation}
        \Phi_{ij}(t) \geq \delta,\;\;\; \Phi_{kj}(t) \geq \delta,
    \end{equation}
    for the column index $j$ that satisfies the scrambling condition for the pair $(i,k)$.
\end{lemma}

\begin{lemma}\label{lemma:right_stochastic}
    $\Phi(t)$ is still right-stochastic, i.e., $\sum_j \Phi_{ij} = 1$.
\end{lemma}

\textbf{Contraction of the Diameter.} Now suppose $i$ and $k$ are any two agents. Then:
\begin{equation}
    x_i(t+T) = \sum_{j=1}^{n} \Phi_{ij}(t) x_j(t),\;\;\;
    x_k(t+T) = \sum_{j=1}^{n} \Phi_{kj}(t) x_j(t)
\end{equation}

We are interested in bounding the difference:
\begin{equation}
    \biggl|x_i(t+T) - x_k(t+T)\biggr| = \left| \sum_{j=1}^{n} \biggl(\Phi_{ij}(t)-\Phi_{kj}(t)\biggr)x_j(t) \right|
\end{equation}
% where $|\cdot|$ denotes the absolute operation.

Let $s_j(t) := \Phi_{ij}(t) - \Phi_{kj}(t)$, then
\begin{equation}\label{eq:difference}
    \biggl|x_i(t+T) - x_k(t+T)\biggr| = \left| \sum_{j=1}^{n} s_j(t)x_j(t) \right|
\end{equation}
Decompose $s_j$ into
\begin{equation}
    \begin{split}
        \text{Positive part:}\;\;\; s^+_j(t) &:= \max(s_j(t),0)\\
        \text{Negative part:}\;\;\; s^-_j(t) &:= \max(-s_j(t),0)\\
    \end{split}
\end{equation}
\begin{lemma}\label{lemma:s_j_decompose}
We have  $s_j(t) = s^+_j(t) - s^-_j(t)\;\; \text{and} \;\; |s_j(t)| = s^+_j(t) + s^-_j(t) $.   
\end{lemma}
Based on Lemma \ref{lemma:s_j_decompose}, we rewrite the RHS of Equation \ref{eq:difference} into
\begin{equation}
    % \left| \sum_{j=1}^{n} \biggl(\Phi_{ij}(t)-\Phi_{kj}(t)\biggr)x_j(t) \right| = 
    \left| \sum_{j=1}^{n} s_j(t)x_j(t) \right| = \left| \sum_{j=1}^{n} s^+_j(t)x_j(t) -\sum_{j=1}^{n} s^-_j(t)x_j(t) \right|
\end{equation}
% Given the lemma 3, we use the fact that for any two probability distributions $p,q$ over the same domain, 
% \begin{equation}
%     \left| \sum_{j=1}^{n} \biggl(p_j-q_j\biggr)x_j \right| \leq D \cdot \left\Vert p-q\right\Vert_1
% \end{equation}
Given the Lemma \ref{lemma:right_stochastic}, we have:
\begin{equation}
    \sum_j(\Phi_{ij}(t) -\Phi_{kj}(t))=0
\end{equation}
For the LHS of Lemma \ref{lemma:s_j_decompose}, summing over all $j$, we have
\begin{equation}\label{eq:s_j_LHS}
    \sum_j s_j(t) = \sum_j s_j^+(t) - \sum_j s^-_j(t) = 0 \;\;\;\; \Rightarrow\;\;\;\;\; \sum_j s_j^+(t) = \sum_j s^-_j(t)
\end{equation}
and
\begin{equation}\label{eq:s_j_RHS}
    \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 = \sum_j \left|s_j(t)\right| = \sum_js^+_j(t) + \sum_j s^-_j(t)
\end{equation}
where $\left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1$ is the norm of $i$-th and $k$-th row of $\Phi(t)$.

Combine Equation \ref{eq:s_j_LHS} and \ref{eq:s_j_RHS}, we have:
\begin{equation}
     \sum_j s_j^+(t) = \sum_j s^-_j(t) = \frac{1}{2} \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1
\end{equation}
Since
\begin{equation}
\begin{split}
    x_j(t) \leq M(t) &\Rightarrow \sum_j s^+_j(t) x_j(t) \leq M(t)\sum_js^+_j(t),\\
    x_j(t) \geq m(t) &\Rightarrow \sum_j s^-_j(t) x_j(t) \geq m(t)\sum_js^-_j(t)
\end{split}
\end{equation}
We have
\begin{equation}\label{eq:s_j_upper}
\begin{split}
    \sum_{j=1}^{n} s^+_j(t)x_j(t) -\sum_{j=1}^{n} s^-_j(t)x_j(t) &\leq M(t)\sum_js^+_j(t) -  m(t)\sum_js^-_j(t)\\
    &= M(t)\cdot \frac{1}{2}\left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 - m(t) \cdot \frac{1}{2}\left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 \\
    &= \frac{1}{2} \biggl(M(t) - m(t)\biggr) \cdot \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 \\
    & = \frac{1}{2} D(t) \cdot \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1
\end{split}
\end{equation}
The same, since
\begin{equation}
\begin{split}
    x_j(t) \leq M(t) &\Rightarrow \sum_j s^-_j(t) x_j(t) \leq M(t)\sum_js^-_j(t),\\
    x_j(t) \geq m(t) &\Rightarrow \sum_j s^+_j(t) x_j(t) \geq m(t)\sum_js^+_j(t)
\end{split}
\end{equation}
We have
\begin{equation}\label{eq:s_j_lower}
\begin{split}
    \sum_{j=1}^{n} s^+_j(t)x_j(t) -\sum_{j=1}^{n} s^-_j(t)x_j(t) &\geq m(t)\sum_js^+_j(t) -  M(t)\sum_js^-_j(t)\\
    &= m(t)\cdot \frac{1}{2}\left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 - M(t) \cdot \frac{1}{2}\left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 \\
    &= -\frac{1}{2} \biggl(M(t) - m(t)\biggr) \cdot \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 \\
    &= -\frac{1}{2} D(t) \cdot \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1
\end{split}
\end{equation}

Noticing $D(t) \geq 0$ and $ \left\Vert \Phi_{i}(t) - \Phi_{k}(t) \right\Vert_1 \geq 0$, we combine Equation \ref{eq:difference} \ref{eq:s_j_upper} \ref{eq:s_j_lower} to get:
\begin{equation}
    \biggl|x_i(t+T) - x_k(t+T)\biggr| \leq \frac{1}{2} D(t) \cdot \left\Vert \Phi_{i}- \Phi_{k}\right\Vert_1
\end{equation}
Since $\Phi(t)$ is scrambling (Lemma \ref{lemma:scrambling}), we have:
\begin{equation}
    \max_{i,k}  \left\Vert \Phi_{i}- \Phi_{k}\right\Vert_1 \leq 1-2\delta
\end{equation}
Therefore,
\begin{equation}
    D(t+T) = \max_{i,k} \biggl|x_i(t+T) - x_j(t+T)\biggr| \leq \frac{1-2\delta}{2}D(t)
\end{equation}
Since $1-2\delta <1$, recursively:
\begin{equation}
    D(t) \leq D(0)\cdot \frac{1-2\delta}{2}^{\lfloor t/T \rfloor}
\end{equation}
which prove the diameter converge to vanish, and therefore the agent opinions exponentially converge to consensus.
% Given the assumption A1 and A2, we conclude $\mathbf{A}(t)$ is scrambling that for every $t$, exist $j$ that for all :
% \begin{equation}
%     \mathbf{A}_{ij}(t) \geq \alpha,\;\;\; \Phi_{kj}(t,t+\tilde{T}) \geq \alpha
% \end{equation}
% which means there’s at least one agent ($j$) that both agents ($i$ and $k$) communicate with directly.

Therefore, unless we employ some technique, such as rewiring, to break or weaken our assumption (A1) and (A2), the oversmoothing will persist in time-varying Laplacian dynamics. This suggests that the common strategy of adaptively updating the Laplacian matrix does not effectively mitigate oversmoothing.

Note: The strong assumption A1 (fixed strong connectivity) can be relaxed to joint strong connectivity, where the connectivity of $\mathcal{G}^{\mathrm{a}}$ is allowed to change over time, as long as there is an interval $T$ such that the union graph
 \begin{equation}
     \mathcal{G}^{\mathrm{a}}_{[t,t+T]} = \cup_{\tau \in [t,t+T]}\mathcal{G}^{\mathrm{a}}(\tau)
 \end{equation}
is strongly connected for all $t$, where $\mathcal{G}^{\mathrm{a}}(\tau)$ denotes the communication graph at time step $\tau$.

\end{proof}
}


==> sections/n_checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper makes four main claims in the abstract/introduction. Namely:
    \begin{enumerate}
        \item Propose an analogy between oversmoothing and opinion consensus. We show this analogy in Section~\ref{sec:analogy} and show the corresponding concepts in Table~\ref{tab:consensus_vs_oversmoothing};
        \item Prove dynamics of recent GNN architectures are equivalent to linear opinion dynamics and therefore exhibits oversmoothing. We show this in Section~\ref{sec:understanding_oversmoothing} and Lemmas proposed in this section are proven in Appendix~\ref{appendix:proof_of_proposition};
        \item Prove that BIMP has greater expressive capacity while resolving oversmoothing. We show this in Section~\ref{section:BIMP} and Lemmas proposed in this section are proven in Appendix~\ref{appendix:proof_of_proposition};
        \item Perform extensive empirical analysis to show that BIMP outperforms baseline models. We show this in Section~\ref{section:experiment}.
    \end{enumerate}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Limitation is provided in Section~\ref{section:conclusion}, where large damping terms $d$ leads to instability during training and therefore limiting the application of large time steps to accelerate training.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All proofs and assumptions to the given Lemmas included in Section~\ref{sec:analogy}, \ref{sec:understanding_oversmoothing}, and \ref{section:BIMP} are given in detail in Appendix~\ref{appendix:proof_of_proposition}. Auxiliary lemmas and proofs are provided in Appendix~\ref{appendix:auxiliary_proofs} to offer deeper insight into the theoretical properties of the BIMP model. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    All the datasets used in Section \ref{section:experiment} are described and summarized in Appendix \ref{appendix:datasets}. All details of the experiments are given in Appendix \ref{appendix:experiment_details}. Specifically, the fine-tuned hyper-parameters for BIMP reported in Table \ref{tab:acc_result_homo} and Table \ref{tab:acc_result_hetero} are listed in Appendix \ref{appendix:fine_tune_homo} and Appendix \ref{appendix:fine_tune_hetero} respectively; the design for 'Classification accuracy' experiment is explained in Appendix \ref{appendix:experiment_depth}; the design for 'Dirichlet energy' experiment is explained in Appendix \ref{appendix:experiment_dirichlet}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Source code will be released upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Hyperparameters for both homo- and heterophilic datasets are included in the Appendix \ref{appendix:fine_tune_homo} and \ref{appendix:fine_tune_hetero}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide standard deviations on all tables and plots. The number of seeds/runs that these are calculated are given in the Appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide computation resource used to run these experiments as well as comparison of space and time complexity. The details are given in the Appendix \ref{appendix:additional_experiment}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research presented in this paper abides by the NeurIPS code of ethics, namely
    \begin{enumerate}
        \item Research involving human subjects or participants: this paper does not include human subjects or participants;
        \item Data-related concerns: the datasets used in this paper are well circulated and adequately cited. No new datasets are part of this submission;
        \item Societal Impact and Potential Harmful Consequences: the authors do not believe that this paper has negative potentials in the field of safety, security, surveillance, deception and harassment, environment, human rights, or bias and fairness. We note that graph neural networks have been extensively applied commercially in networks systems such as recommendation algorithms and therefore may negatively discriminate certain demographic groups determined by aspects such as (and not limited to) finance and geography. We however note that the proposed method does not enables such behavior beyond what existing methods are able to.
    \end{enumerate}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: By building the analogy between graph neural networks and opinion dynamics models, we present a novel continuous-depth graph neural networks to tackle the oversmoothing issue and enable us to build a deep model with enhanced expressive capacity. The improved expressivity can lead to some breakthroughs in various domains such as drug discovery, protein prediction and multi-agent robots control, where we don't anticipate the negative societal impacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Release of pretrained models and datasets is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Release of assets is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Release of assets is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Research with human subjects and crowdsourcing is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Research with human subjects and crowdsourcing is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Research involving LLMs is not part of this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}
